Low Dynamic Range for RIS-aided Bistatic Integrated Sensing and Communication

The following paper presents a reconfigurable intelligent surface (RIS)-aided integrated sensing and communication (ISAC) system model scenario, where a base station communicates with a user, and a bi-static sensing unit, i.e. the passive radar (PR), senses targets using downlink signals. Given that the RIS aids with communication and sensing tasks, this paper introduces new interfering paths that can overwhelm the PR with unnecessarily high power, namely the path interference (PI), \textit{which is itself a combination of two interfering paths, the direct path interference (DPI) and the reflected path interference (RPI)}. For this, we formulate an optimization framework that allows the system to carry on with its ISAC tasks, through analog space-time beamforming at the sensing unit, in collaboration with RIS phase shift and statistical transmit covariance matrix optimization, while minimizing the PI power. As the proposed optimization problem is non-convex, we tailor a block-cyclic coordinate descent (BCCD) method to decouple the non-convex sub-problem from the convex one. A Riemannian conjugate gradient method is devised to generate the RIS and PR space-time beamforming phase shifts per BCCD iteration, while the convex sub-problem is solved via off-the-shelf solvers. Simulation results demonstrate the effectiveness of the proposed solver when compared with benchmarking ones.

==> Actions/eq-main-subproblem-3.tex <==
	(\mathcal{P}_2)\left\{\begin{aligned}
\min _{\boldsymbol{R}_{ss}} \quad  & \operatorname{tr}(
	\boldsymbol{A}_c^H (\phi) 
	{\pmb{w}}
	{\pmb{w}}^H\boldsymbol{A}_c(\phi) \pmb{R}_{ss} ) \\
\rm { s.t. } \quad  & 
\operatorname{tr}(\boldsymbol{R}_{ss} \boldsymbol{H}_c^{H}(\boldsymbol{\phi}) \boldsymbol{H}_c(\boldsymbol{\phi})) \geq \gamma_{\rm{comm}}M_r L \sigma_c^2, \\
& \operatorname{tr}(
	\boldsymbol{A}_r^H (\phi) 
	{\pmb{w}}
	{\pmb{w}}^H\boldsymbol{A}_r(\phi) \pmb{R}_{ss} - \gamma_{\rm{sense}}\sigma_r^2 \pmb{w}\pmb{w}^H
	- \gamma_{\rm{sense}}\boldsymbol{A}_c^H (\phi) 
	{\pmb{w}}
	{\pmb{w}}^H\boldsymbol{A}_c(\phi) \pmb{R}_{ss}
	- \gamma_{\rm{sense}}\boldsymbol{A}_o^H (\phi) 
	{\pmb{w}}
	{\pmb{w}}^H\boldsymbol{A}_o(\phi) \pmb{R}_{ss} ) \geq 0, \\
& \operatorname{tr}\left(\boldsymbol{R}_{ss}\right)=P_B, \quad \boldsymbol{R}_{ss} \succeq \pmb{0}. \\
\end{aligned}\right.

==> Actions/summaryofactions.tex <==
We would like to thank the editor for the comments. In light of the reviewers comments, we summarize our action items as follows:
\begin{itemize}
	\item We have expanded the open challenges section to add more context related to all open challenges including scalability, efficacy, imperfect \ac{CSI}, \ac{ADC} optimization, and near-field case.
	\item For the imperfect \ac{CSI} in Section \ref{subsec:imperfect-csi-challenge} of the updated manuscript, we included guidelines on how to proceed if the \ac{BS}, \ac{RIS} and \ac{PR} have access to imperfect channel state knowledge.
	\item We have reformatted the figures to make them less crowded and more readable as per the reviewer's comments.
	\item We have included how the \ac{PR} could communicate target detection results back to the central processing unit.
	\item We have included more state of the art work on \ac{RIS} applied on \ac{ISAC}.
	\item We have added obstacles and interferers in the system model and adapted the optimization problems accordingly.
	\item We have performed complexity analysis of the proposed methods in Section \ref{subsec:complexity-analysis} of the updated manuscript.
	\item We have rewritten the Conclusions section.
	\item We have corrected typos and defined symbols that weren't defined in the first version of this manuscript.
\end{itemize}

==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    if (!($root_filename eq $_[0]))
    {
        # FOR PDFLATEX
        system( "latexmk -cd -pdf \"$_[0]\"" );

        # FOR LATEX+DVIPDF
        # system( "latexmk -cd \"$_[0]\"" );

        # FOR XELATEX
        # system( "latexmk -cd -xelatex \"$_[0]\"" );
        
        # FOR LUALATEX
        # system( "latexmk -cd -lualatex \"$_[0]\"" );
   }
}
